Improving Web Content Blocking With Event-Loop-Turn Granularity JavaScript Signatures

Content blocking is an important part of a performant, user-serving, privacy respecting web. Most content blockers build trust labels over URLs. While useful, this approach has well understood shortcomings. Attackers may avoid detection by changing URLs or domains, bundling unwanted code with benign code, or inlining code in pages. The common flaw in existing approaches is that they evaluate code based on its delivery mechanism, not its behavior. In this work we address this problem with a system for generating signatures of the privacy-and-security relevant behavior of executed JavaScript. Our system considers script behavior during each turn on the JavaScript event loop. Focusing on event loop turns allows us to build signatures that are robust against code obfuscation, code bundling, URL modification, and other common evasions, as well as handle unique aspects of web applications. This work makes the following contributions to improving content blocking: First, implement a novel system to build per-event-loop-turn signatures of JavaScript code by instrumenting the Blink and V8 runtimes. Second, we apply these signatures to measure filter list evasion, by using EasyList and EasyPrivacy as ground truth and finding other code that behaves identically. We build ~2m signatures of privacy-and-security behaviors from 11,212 unique scripts blocked by filter lists, and find 3,589 more unique scripts including the same harmful code, affecting 12.48% of websites measured. Third, we taxonomize common filter list evasion techniques. Finally, we present defenses; filter list additions where possible, and a proposed, signature based system in other cases. We share the implementation of our signature-generation system, the dataset from applying our system to the Alexa 100K, and 586 AdBlock Plus compatible filter list rules to block instances of currently blocked code being moved to new URLs.

==> Makefile <==
extensions_to_clean := out aux log bbl blg fls fdb_latexmk glg gls lof glo glsdefs lot toc dvi ist acn acr synctex.gz alg xdy

all: main

clean:
	@if [[ -f main.pdf ]]; then \
		rm main.pdf;\
	fi;
	@for extension in $(extensions_to_clean); do \
		find . -type f -name "*.$$extension" -delete;\
	done;
	@rm -f diff.*

main:
	latexmk -bibtex -pdf main
	pdflatex -bibtex -interaction=batchmode main

diff:
	latexmk -bibtex -pdf diff
	pdflatex -bibtex -interaction=batchmode diff


==> figures/alexa_top10k-100k.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=.8\columnwidth]{figures/alexa_top10k-100k_render.pdf}
  \caption{Total number of evaded scripts per website, for Alexa top 10K - 100K.}
  \label{fig:alexa-10k-100k-evasion}
\end{figure}


==> figures/alexa_top1k-10k.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=.8\columnwidth]{figures/alexa_top1k-10k_render.pdf}
  \caption{Total number of evaded scripts per website, for Alexa top 1K - 10K.}
  \label{fig:alexa-1k-10k-evasion}
\end{figure}


==> figures/alexa_top1k.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=.8\columnwidth]{figures/alexa_top1k_render.pdf}
  \caption{Total number of evaded scripts per website, for Alexa top 1K.}
  \label{fig:alexa-1k-evasion}
\end{figure}


==> figures/theoatmeal-com.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/theoatmeal-com_render.pdf}
  \caption{PageGraph recorded execution of rendering \url{https://theoatmeal.com},
    showing the attribution of page events to their relevant actor.  The
    circled subsection is the script fetched from \url{https://ssl.google-analytics.com/ga.js}.}
  \label{fig:theoatmeal-com}
\end{figure*}


==> tables/instrumentation-points.tex <==
\begin{table}
  \begin{tabular}{l}
    \toprule
      DOM Events \\
    \midrule
      \ctab{} node creation \\
      \ctab{} node insertion \\
      \ctab{} node deletion \\
      \ctab{} node modification \\
      \ctab{} script executions \\
      \ctab{} frame creations \\
      \ctab{} operations in local (i.e. same domain) frames \\
    \midrule
      Network requests \\
    \midrule
      \ctab{} AJAX API \\
      \ctab{} Fetch API \\
      \ctab{} DOM-related (e.g. \texttt{<img scr=X>}) \\
    \midrule
      \JS{} Builtin APIs \\
    \midrule
      \ctab{} date APIs \\
      \ctab{} timer APIs \\
      \ctab{} event registrations \\
    \midrule
      Web APIs \\
    \midrule
      \ctab{} storage APIs (\\
      \ctab{} \ctab{} \texttt{document.cookie}, \texttt{localStorage}, \texttt{sessionStorage}) \\
      \ctab{} APIs used by browser fingerprinting scripts (e.g. \\
      \ctab{} \ctab{} \texttt{navigator.\{platform, userAgent, language\}, etc}, \\
      \ctab{} \ctab{} \texttt{screen.\{height, width, colorDepth, pixelDepth\}}) \\
    \bottomrule
  \end{tabular}
  \caption{A complete list of events that are instrumented by PageGraph}.
  \label{table:instrumentation-points}
\end{table}

==> tables/signature_stats_summary.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{lrr}
    \toprule
     & URLs & Domains \\
    \midrule
    Blocked & \NumBlockedFingerprintedScriptURLs{} & \NumDomainsHostingBlockedFingerprintedScripts\\
    Evaded (exp) & \NumNewFingerprintedScriptURLs{} & \NumDomainsHostingNewFingerprintedScripts \\
    Evaded (non-exp) & \NumNewNotExceptFingerprintedScriptURLs{} & \NumDomainsHostingNewNotExceptFingerprintedScripts \\
    Total & \NumFingerprintedScriptURLs{} & \NumDomainsHostingFingerprintedScripts{} \\
    \bottomrule
    \end{tabular}
    \caption{Summary of the number of script URLs matched by Page Graph signatures and the domains they are hosted on, broken down by 1) whether they are blocked by EL/EP, and if not blocked, 2) whether it is due to exception rules (exp) or not (non-exp).}
    \label{tab:script_urls_domains_summary}
    %\vspace{-10pt}
\end{figure}
